Multi-Task Classification Hypothesis Space with Improved Generalization Bounds

This paper presents a RKHS, in general, of vector-valued functions intended to be used as hypothesis space for multi-task classification. It extends similar hypothesis spaces that have previously considered in the literature. Assuming this space, an improved Empirical Rademacher Complexity-based generalization bound is derived. The analysis is itself extended to an MKL setting. The connection between the proposed hypothesis space and a Group-Lasso type regularizer is discussed. Finally, experimental results, with some SVM-based Multi-Task Learning problems, underline the quality of the derived bounds and validate the paper's analysis.

==> TitleAuthors.tex <==
\title{Multi-Task Classification Hypothesis Space with Improved Generalization Bounds}

\author{Cong Li         \and
        Michael Georgiopoulos \and
        Georgios C. Anagnostopoulos
}

%\authorrunning{Short form of author list} % if too long for running head

\institute{Cong Li \at
              Department of Electrical Engineering and Computer Science, \\
							University of Central Florida, Florida, 32816, USA  \\
              \email{licong@knights.ucf.edu}           %  \\
%             \emph{Present address:} of F. Author  %  if needed
           \and
           Michael Georgiopoulos \at
              Department of Electrical Engineering and Computer Science, \\
							University of Central Florida, Florida, 32816, USA  \\
              \email{michaelg@ucf.edu}           %  \\
					 \and
           Georgios C. Anagnostopoulos \at
              Department of Department of Electrical \& Computer Engineering, \\
							Florida Institute of Technology, Melbourne, 32901, USA  \\
              \email{georgio@fit.edu}           %  \\
}
